Geometry and Symmetry in Short-and-Sparse Deconvolution

We study the $\textit{Short-and-Sparse (SaS) deconvolution}$ problem of recovering a short signal $\mathbf a_0$ and a sparse signal $\mathbf x_0$ from their convolution. We propose a method based on nonconvex optimization, which under certain conditions recovers the target short and sparse signals, up to a signed shift symmetry which is intrinsic to this model. This symmetry plays a central role in shaping the optimization landscape for deconvolution. We give a $\textit{regional analysis}$, which characterizes this landscape geometrically, on a union of subspaces. Our geometric characterization holds when the length-$p_0$ short signal $\mathbf a_0$ has shift coherence $\mu$, and $\mathbf x_0$ follows a random sparsity model with sparsity rate $\theta \in \Bigl[\frac{c_1}{p_0}, \frac{c_2}{p_0\sqrt\mu + \sqrt{p_0}}\Bigr]\cdot\frac{1}{\log^2p_0}$. Based on this geometry, we give a provable method that successfully solves SaS deconvolution with high probability.

==> sections/saddle_plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

\begin{axis}[%
width=1.5in,
height=1.25in,
at={(-1.5in,0in)},
scale only axis,
xmin=0.2,
xmax=0.9,
xtick={\empty},
tick align=outside,
ymin=-0.3,
ymax=0.3,
ytick={\empty},
zmin=12,
zmax=22,
ztick={\empty},
view={45}{50},
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
axis z line*=left,
legend style={at={(0.03,0.03)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]

\addplot3[%
surf,
shader=flat corner, z buffer=sort, colormap={mymap}{[1pt] rgb(0pt)=(0.2422,0.1504,0.6603); rgb(1pt)=(0.25039,0.164995,0.707614); rgb(2pt)=(0.257771,0.181781,0.751138); rgb(3pt)=(0.264729,0.197757,0.795214); rgb(4pt)=(0.270648,0.214676,0.836371); rgb(5pt)=(0.275114,0.234238,0.870986); rgb(6pt)=(0.2783,0.255871,0.899071); rgb(7pt)=(0.280333,0.278233,0.9221); rgb(8pt)=(0.281338,0.300595,0.941376); rgb(9pt)=(0.281014,0.322757,0.957886); rgb(10pt)=(0.279467,0.344671,0.971676); rgb(11pt)=(0.275971,0.366681,0.982905); rgb(12pt)=(0.269914,0.3892,0.9906); rgb(13pt)=(0.260243,0.412329,0.995157); rgb(14pt)=(0.244033,0.435833,0.998833); rgb(15pt)=(0.220643,0.460257,0.997286); rgb(16pt)=(0.196333,0.484719,0.989152); rgb(17pt)=(0.183405,0.507371,0.979795); rgb(18pt)=(0.178643,0.528857,0.968157); rgb(19pt)=(0.176438,0.549905,0.952019); rgb(20pt)=(0.168743,0.570262,0.935871); rgb(21pt)=(0.154,0.5902,0.9218); rgb(22pt)=(0.146029,0.609119,0.907857); rgb(23pt)=(0.138024,0.627629,0.89729); rgb(24pt)=(0.124814,0.645929,0.888343); rgb(25pt)=(0.111252,0.6635,0.876314); rgb(26pt)=(0.0952095,0.679829,0.859781); rgb(27pt)=(0.0688714,0.694771,0.839357); rgb(28pt)=(0.0296667,0.708167,0.816333); rgb(29pt)=(0.00357143,0.720267,0.7917); rgb(30pt)=(0.00665714,0.731214,0.766014); rgb(31pt)=(0.0433286,0.741095,0.73941); rgb(32pt)=(0.0963952,0.75,0.712038); rgb(33pt)=(0.140771,0.7584,0.684157); rgb(34pt)=(0.1717,0.766962,0.655443); rgb(35pt)=(0.193767,0.775767,0.6251); rgb(36pt)=(0.216086,0.7843,0.5923); rgb(37pt)=(0.246957,0.791795,0.556743); rgb(38pt)=(0.290614,0.79729,0.518829); rgb(39pt)=(0.340643,0.8008,0.478857); rgb(40pt)=(0.3909,0.802871,0.435448); rgb(41pt)=(0.445629,0.802419,0.390919); rgb(42pt)=(0.5044,0.7993,0.348); rgb(43pt)=(0.561562,0.794233,0.304481); rgb(44pt)=(0.617395,0.787619,0.261238); rgb(45pt)=(0.671986,0.779271,0.2227); rgb(46pt)=(0.7242,0.769843,0.191029); rgb(47pt)=(0.773833,0.759805,0.16461); rgb(48pt)=(0.820314,0.749814,0.153529); rgb(49pt)=(0.863433,0.7406,0.159633); rgb(50pt)=(0.903543,0.733029,0.177414); rgb(51pt)=(0.939257,0.728786,0.209957); rgb(52pt)=(0.972757,0.729771,0.239443); rgb(53pt)=(0.995648,0.743371,0.237148); rgb(54pt)=(0.996986,0.765857,0.219943); rgb(55pt)=(0.995205,0.789252,0.202762); rgb(56pt)=(0.9892,0.813567,0.188533); rgb(57pt)=(0.978629,0.838629,0.176557); rgb(58pt)=(0.967648,0.8639,0.16429); rgb(59pt)=(0.96101,0.889019,0.153676); rgb(60pt)=(0.959671,0.913457,0.142257); rgb(61pt)=(0.962795,0.937338,0.12651); rgb(62pt)=(0.969114,0.960629,0.106362); rgb(63pt)=(0.9769,0.9839,0.0805)}, mesh/rows=31, forget plot]
table[row sep=crcr, point meta=\thisrow{c}] {%
%
x	y	z	c\\
0.2	-0.3	18.2601701512401	18.2601701512401\\
0.22	-0.3	18.6360691501232	18.6360691501232\\
0.24	-0.3	18.9906070806165	18.9906070806165\\
0.26	-0.3	19.3221339542314	19.3221339542314\\
0.28	-0.3	19.6298045170094	19.6298045170094\\
0.3	-0.3	19.9128464714294	19.9128464714294\\
0.32	-0.3	20.1703735119586	20.1703735119586\\
0.34	-0.3	20.4011117829218	20.4011117829218\\
0.36	-0.3	20.604198959811	20.604198959811\\
0.38	-0.3	20.7794168350781	20.7794168350781\\
0.4	-0.3	20.9266894223251	20.9266894223251\\
0.42	-0.3	21.0458529379139	21.0458529379139\\
0.44	-0.3	21.1369684576826	21.1369684576826\\
0.46	-0.3	21.1999825341474	21.1999825341474\\
0.48	-0.3	21.2345501381106	21.2345501381106\\
0.5	-0.3	21.2404921720053	21.2404921720053\\
0.52	-0.3	21.2180317223302	21.2180317223302\\
0.54	-0.3	21.1674597500758	21.1674597500758\\
0.56	-0.3	21.0890408395686	21.0890408395686\\
0.58	-0.3	20.9828172670417	20.9828172670417\\
0.6	-0.3	20.8488656223276	20.8488656223276\\
0.62	-0.3	20.6875912652533	20.6875912652533\\
0.64	-0.3	20.4994958586963	20.4994958586963\\
0.66	-0.3	20.2855402703285	20.2855402703285\\
0.68	-0.3	20.0466117267452	20.0466117267452\\
0.7	-0.3	19.7833475499929	19.7833475499929\\
0.72	-0.3	19.4963512094594	19.4963512094594\\
0.74	-0.3	19.1866362006746	19.1866362006746\\
0.76	-0.3	18.8549367105908	18.8549367105908\\
0.78	-0.3	18.5021524324869	18.5021524324869\\
0.8	-0.3	18.129422603981	18.129422603981\\
0.2	-0.28	17.5950990373983	17.5950990373983\\
0.22	-0.28	17.9728473298499	17.9728473298499\\
0.24	-0.28	18.3291670070882	18.3291670070882\\
0.26	-0.28	18.6623763511002	18.6623763511002\\
0.28	-0.28	18.9716132766062	18.9716132766062\\
0.3	-0.28	19.2561255973013	19.2561255973013\\
0.32	-0.28	19.5150214845373	19.5150214845373\\
0.34	-0.28	19.7469984334768	19.7469984334768\\
0.36	-0.28	19.9512358719663	19.9512358719663\\
0.38	-0.28	20.1275228528103	20.1275228528103\\
0.4	-0.28	20.275683981184	20.275683981184\\
0.42	-0.28	20.3956168766599	20.3956168766599\\
0.44	-0.28	20.4873485772991	20.4873485772991\\
0.46	-0.28	20.5507774673684	20.5507774673684\\
0.48	-0.28	20.5855911009217	20.5855911009217\\
0.5	-0.28	20.5916247712227	20.5916247712227\\
0.52	-0.28	20.5691186892885	20.5691186892885\\
0.54	-0.28	20.5182632045626	20.5182632045626\\
0.56	-0.28	20.4393781149756	20.4393781149756\\
0.58	-0.28	20.3326196727317	20.3326196727317\\
0.6	-0.28	20.1980020457118	20.1980020457118\\
0.62	-0.28	20.0359034660404	20.0359034660404\\
0.64	-0.28	19.8469036422207	19.8469036422207\\
0.66	-0.28	19.6318828513505	19.6318828513505\\
0.68	-0.28	19.3918269485713	19.3918269485713\\
0.7	-0.28	19.1272810072229	19.1272810072229\\
0.72	-0.28	18.8388826822693	18.8388826822693\\
0.74	-0.28	18.5276568618523	18.5276568618523\\
0.76	-0.28	18.1943951362412	18.1943951362412\\
0.78	-0.28	17.8399756452923	17.8399756452923\\
0.8	-0.28	17.4654807030237	17.4654807030237\\
0.2	-0.26	16.9716579059459	16.9716579059459\\
0.22	-0.26	17.3511269514874	17.3511269514874\\
0.24	-0.26	17.7091056312384	17.7091056312384\\
0.26	-0.26	18.0439169138966	18.0439169138966\\
0.28	-0.26	18.3546114160256	18.3546114160256\\
0.3	-0.26	18.6405012621892	18.6405012621892\\
0.32	-0.26	18.9006266206526	18.9006266206526\\
0.34	-0.26	19.1337354312721	19.1337354312721\\
0.36	-0.26	19.3390838318301	19.3390838318301\\
0.38	-0.26	19.51638489541	19.51638489541\\
0.4	-0.26	19.6654090963704	19.6654090963704\\
0.42	-0.26	19.7860853947712	19.7860853947712\\
0.44	-0.26	19.8784052007564	19.8784052007564\\
0.46	-0.26	19.9422215993929	19.9422215993929\\
0.48	-0.26	19.9772632870949	19.9772632870949\\
0.5	-0.26	19.9834037537941	19.9834037537941\\
0.52	-0.26	19.9608714382685	19.9608714382685\\
0.54	-0.26	19.9097871388489	19.9097871388489\\
0.56	-0.26	19.8304820389437	19.8304820389437\\
0.58	-0.26	19.7231648209008	19.7231648209008\\
0.6	-0.26	19.5879104401673	19.5879104401673\\
0.62	-0.26	19.42506734474	19.42506734474\\
0.64	-0.26	19.2351884423346	19.2351884423346\\
0.66	-0.26	19.0191932223812	19.0191932223812\\
0.68	-0.26	18.7780782664899	18.7780782664899\\
0.7	-0.26	18.5123327592538	18.5123327592538\\
0.72	-0.26	18.222588409242	18.222588409242\\
0.74	-0.26	17.9099287780531	17.9099287780531\\
0.76	-0.26	17.575205070059	17.575205070059\\
0.78	-0.26	17.2192844664575	17.2192844664575\\
0.8	-0.26	16.8432127385842	16.8432127385842\\
0.2	-0.24	16.3905377265215	16.3905377265215\\
0.22	-0.24	16.7716071368739	16.7716071368739\\
0.24	-0.24	17.1311088128207	17.1311088128207\\
0.26	-0.24	17.4674052911963	17.4674052911963\\
0.28	-0.24	17.7794835266199	17.7794835266199\\
0.3	-0.24	18.06665507152	18.06665507152\\
0.32	-0.24	18.3278855028091	18.3278855028091\\
0.34	-0.24	18.5620440380287	18.5620440380287\\
0.36	-0.24	18.7684603177796	18.7684603177796\\
0.38	-0.24	18.946717956406	18.946717956406\\
0.4	-0.24	19.0965841675918	19.0965841675918\\
0.42	-0.24	19.2179540776577	19.2179540776577\\
0.44	-0.24	19.3108157077615	19.3108157077615\\
0.46	-0.24	19.3750062917685	19.3750062917685\\
0.48	-0.24	19.4102786632081	19.4102786632081\\
0.5	-0.24	19.4165403224433	19.4165403224433\\
0.52	-0.24	19.3939784892196	19.3939784892196\\
0.54	-0.24	19.3427098311715	19.3427098311715\\
0.56	-0.24	19.2630458818262	19.2630458818262\\
0.58	-0.24	19.1551693187954	19.1551693187954\\
0.6	-0.24	19.0192886405181	19.0192886405181\\
0.62	-0.24	18.8557625197197	18.8557625197197\\
0.64	-0.24	18.6650620845603	18.6650620845603\\
0.66	-0.24	18.4481689985407	18.4481689985407\\
0.68	-0.24	18.2060609370808	18.2060609370808\\
0.7	-0.24	17.9391891336641	17.9391891336641\\
0.72	-0.24	17.6481770991819	17.6481770991819\\
0.74	-0.24	17.334165094564	17.334165094564\\
0.76	-0.24	16.9980845556271	16.9980845556271\\
0.78	-0.24	16.6408169492892	16.6408169492892\\
0.8	-0.24	16.2633281153476	16.2633281153476\\
0.2	-0.22	15.8524133419012	15.8524133419012\\
0.22	-0.22	16.2349379045316	16.2349379045316\\
0.24	-0.22	16.595828312912	16.595828312912\\
0.26	-0.22	16.9335033489105	16.9335033489105\\
0.28	-0.22	17.246872336677	17.246872336677\\
0.3	-0.22	17.5352232429005	17.5352232429005\\
0.32	-0.22	17.7974527412037	17.7974527412037\\
0.34	-0.22	18.0326022679024	18.0326022679024\\
0.36	-0.22	18.2400311952007	18.2400311952007\\
0.38	-0.22	18.4192027189426	18.4192027189426\\
0.4	-0.22	18.5698595015177	18.5698595015177\\
0.42	-0.22	18.6918653012995	18.6918653012995\\
0.44	-0.22	18.7852437233332	18.7852437233332\\
0.46	-0.22	18.8498018422069	18.8498018422069\\
0.48	-0.22	18.8853114710858	18.8853114710858\\
0.5	-0.22	18.8916928863053	18.8916928863053\\
0.52	-0.22	18.8691104938729	18.8691104938729\\
0.54	-0.22	18.817687064661	18.817687064661\\
0.56	-0.22	18.7376914635958	18.7376914635958\\
0.58	-0.22	18.6292974406963	18.6292974406963\\
0.6	-0.22	18.49280730181	18.49280730181\\
0.62	-0.22	18.3286145394682	18.3286145394682\\
0.64	-0.22	18.1371599657044	18.1371599657044\\
0.66	-0.22	17.9194569081982	17.9194569081982\\
0.68	-0.22	17.6764021288452	17.6764021288452\\
0.7	-0.22	17.4084893819994	17.4084893819994\\
0.72	-0.22	17.1163351867754	17.1163351867754\\
0.74	-0.22	16.8010797682032	16.8010797682032\\
0.76	-0.22	16.4637707131781	16.4637707131781\\
0.78	-0.22	16.1052790275818	16.1052790275818\\
0.8	-0.22	15.7264769709355	15.7264769709355\\
0.2	-0.2	15.3579240268953	15.3579240268953\\
0.22	-0.2	15.7417508465759	15.7417508465759\\
0.24	-0.2	16.1039085236336	16.1039085236336\\
0.26	-0.2	16.4428559409254	16.4428559409254\\
0.28	-0.2	16.7574003740698	16.7574003740698\\
0.3	-0.2	17.0467892231562	17.0467892231562\\
0.32	-0.2	17.3099598759611	17.3099598759611\\
0.34	-0.2	17.5460466271621	17.5460466271621\\
0.36	-0.2	17.7544238287382	17.7544238287382\\
0.38	-0.2	17.9344544255829	17.9344544255829\\
0.4	-0.2	18.0858510560588	18.0858510560588\\
0.42	-0.2	18.2084690771897	18.2084690771897\\
0.44	-0.2	18.3023325782097	18.3023325782097\\
0.46	-0.2	18.3672511914894	18.3672511914894\\
0.48	-0.2	18.4030124157867	18.4030124157867\\
0.5	-0.2	18.4095141095484	18.4095141095484\\
0.52	-0.2	18.3868950942513	18.3868950942513\\
0.54	-0.2	18.3353393746161	18.3353393746161\\
0.56	-0.2	18.2550135032819	18.2550135032819\\
0.58	-0.2	18.1461420850729	18.1461420850729\\
0.6	-0.2	18.009100857768	18.009100857768\\
0.62	-0.2	17.8442420379689	17.8442420379689\\
0.64	-0.2	17.6520938155643	17.6520938155643\\
0.66	-0.2	17.4336687127795	17.4336687127795\\
0.68	-0.2	17.1897463202	17.1897463202\\
0.7	-0.2	16.9208672421138	16.9208672421138\\
0.72	-0.2	16.6276961113401	16.6276961113401\\
0.74	-0.2	16.3113219373634	16.3113219373634\\
0.76	-0.2	15.9729042132136	15.9729042132136\\
0.78	-0.2	15.6132906558146	15.6132906558146\\
0.8	-0.2	15.2332818619006	15.2332818619006\\
0.2	-0.18	14.9076312360896	14.9076312360896\\
0.22	-0.18	15.2926163013054	15.2926163013054\\
0.24	-0.18	15.6559386169152	15.6559386169152\\
0.26	-0.18	15.9960404447665	15.9960404447665\\
0.28	-0.18	16.3116319353022	16.3116319353022\\
0.3	-0.18	16.6019275953768	16.6019275953768\\
0.32	-0.18	16.8659791244005	16.8659791244005\\
0.34	-0.18	17.102914773552	17.102914773552\\
0.36	-0.18	17.3121678788272	17.3121678788272\\
0.38	-0.18	17.4930184813605	17.4930184813605\\
0.4	-0.18	17.6451087513689	17.6451087513689\\
0.42	-0.18	17.768349637577	17.768349637577\\
0.44	-0.18	17.8626607472715	17.8626607472715\\
0.46	-0.18	17.9279043501092	17.9279043501092\\
0.48	-0.18	17.9639342632245	17.9639342632245\\
0.5	-0.18	17.9705519878681	17.9705519878681\\
0.52	-0.18	17.9478882402966	17.9478882402966\\
0.54	-0.18	17.8962013353756	17.8962013353756\\
0.56	-0.18	17.8155637237448	17.8155637237448\\
0.58	-0.18	17.7062699164983	17.7062699164983\\
0.6	-0.18	17.5687077076672	17.5687077076672\\
0.62	-0.18	17.4032218642726	17.4032218642726\\
0.64	-0.18	17.2104491066003	17.2104491066003\\
0.66	-0.18	16.9913601255495	16.9913601255495\\
0.68	-0.18	16.7466738335661	16.7466738335661\\
0.7	-0.18	16.476907731885	16.476907731885\\
0.72	-0.18	16.182816260337	16.182816260337\\
0.74	-0.18	15.8654595966165	15.8654595966165\\
0.76	-0.18	15.5260407287154	15.5260407287154\\
0.78	-0.18	15.1654146523836	15.1654146523836\\
0.8	-0.18	14.7843057138763	14.7843057138763\\
0.2	-0.16	14.5020455147563	14.5020455147563\\
0.22	-0.16	14.8880790338963	14.8880790338963\\
0.24	-0.16	15.2524318516397	15.2524318516397\\
0.26	-0.16	15.5935465526925	15.5935465526925\\
0.28	-0.16	15.9100838970902	15.9100838970902\\
0.3	-0.16	16.2011890135449	16.2011890135449\\
0.32	-0.16	16.4660139021557	16.4660139021557\\
0.34	-0.16	16.7037160834938	16.7037160834938\\
0.36	-0.16	16.9137574670191	16.9137574670191\\
0.38	-0.16	17.0953676540077	17.0953676540077\\
0.4	-0.16	17.2481254681689	17.2481254681689\\
0.42	-0.16	17.3719469167337	17.3719469167337\\
0.44	-0.16	17.4666906115034	17.4666906115034\\
0.46	-0.16	17.5322625099365	17.5322625099365\\
0.48	-0.16	17.568532052346	17.568532052346\\
0.5	-0.16	17.5752643467509	17.5752643467509\\
0.52	-0.16	17.5525675257274	17.5525675257274\\
0.54	-0.16	17.5007326373041	17.5007326373041\\
0.56	-0.16	17.4198363218654	17.4198363218654\\
0.58	-0.16	17.3101800248511	17.3101800248511\\
0.6	-0.16	17.1721380399136	17.1721380399136\\
0.62	-0.16	17.0060724610393	17.0060724610393\\
0.64	-0.16	16.812740017578	16.812740017578\\
0.66	-0.16	16.5930471776484	16.5930471776484\\
0.68	-0.16	16.3476590582303	16.3476590582303\\
0.7	-0.16	16.0771197827162	16.0771197827162\\
0.72	-0.16	15.7821735848487	15.7821735848487\\
0.74	-0.16	15.4639704073174	15.4639704073174\\
0.76	-0.16	15.1236835031645	15.1236835031645\\
0.78	-0.16	14.7621395467133	14.7621395467133\\
0.8	-0.16	14.3800370847763	14.3800370847763\\
0.2	-0.14	14.1416479195532	14.1416479195532\\
0.22	-0.14	14.5286054319625	14.5286054319625\\
0.24	-0.14	14.8938528080944	14.8938528080944\\
0.26	-0.14	15.2358390140438	15.2358390140438\\
0.28	-0.14	15.5532177527863	15.5532177527863\\
0.3	-0.14	15.8450310981325	15.8450310981325\\
0.32	-0.14	16.110514122963	16.110514122963\\
0.34	-0.14	16.3489076130188	16.3489076130188\\
0.36	-0.14	16.5596259509011	16.5596259509011\\
0.38	-0.14	16.7419373721292	16.7419373721292\\
0.4	-0.14	16.8953365214061	16.8953365214061\\
0.42	-0.14	17.0196715714792	17.0196715714792\\
0.44	-0.14	17.1148554910468	17.1148554910468\\
0.46	-0.14	17.1807556183721	17.1807556183721\\
0.48	-0.14	17.2172205330967	17.2172205330967\\
0.5	-0.14	17.224063732732	17.224063732732\\
0.52	-0.14	17.2013456259809	17.2013456259809\\
0.54	-0.14	17.1493974528494	17.1493974528494\\
0.56	-0.14	17.0682967102119	17.0682967102119\\
0.58	-0.14	16.9583301184214	16.9583301184214\\
0.6	-0.14	16.8198352384512	16.8198352384512\\
0.62	-0.14	16.6532522316023	16.6532522316023\\
0.64	-0.14	16.4594217816472	16.4594217816472\\
0.66	-0.14	16.239178720522	16.239178720522\\
0.68	-0.14	15.9931741427057	15.9931741427057\\
0.7	-0.14	15.7219374971566	15.7219374971566\\
0.72	-0.14	15.4262446089473	15.4262446089473\\
0.74	-0.14	15.1073021963058	15.1073021963058\\
0.76	-0.14	14.7662611489276	14.7662611489276\\
0.78	-0.14	14.4039106394325	14.4039106394325\\
0.8	-0.14	14.020937786868	14.020937786868\\
0.2	-0.12	13.8268626893531	13.8268626893531\\
0.22	-0.12	14.2146264662076	14.2146264662076\\
0.24	-0.12	14.5806241621386	14.5806241621386\\
0.26	-0.12	14.9233414953131	14.9233414953131\\
0.28	-0.12	15.2414349618929	15.2414349618929\\
0.3	-0.12	15.5338724100857	15.5338724100857\\
0.32	-0.12	15.7999010840132	15.7999010840132\\
0.34	-0.12	16.0388800114234	16.0388800114234\\
0.36	-0.12	16.2501897183971	16.2501897183971\\
0.38	-0.12	16.4331368438604	16.4331368438604\\
0.4	-0.12	16.5871070994063	16.5871070994063\\
0.42	-0.12	16.7119098216169	16.7119098216169\\
0.44	-0.12	16.8075243903979	16.8075243903979\\
0.46	-0.12	16.8737467246329	16.8737467246329\\
0.48	-0.12	16.9104154256905	16.9104154256905\\
0.5	-0.12	16.9173684750453	16.9173684750453\\
0.52	-0.12	16.8946515766868	16.8946515766868\\
0.54	-0.12	16.8426184485859	16.8426184485859\\
0.56	-0.12	16.761345921197	16.761345921197\\
0.58	-0.12	16.6511118314394	16.6511118314394\\
0.6	-0.12	16.5122488972641	16.5122488972641\\
0.62	-0.12	16.3452113130336	16.3452113130336\\
0.64	-0.12	16.1509237067301	16.1509237067301\\
0.66	-0.12	15.9301747264511	15.9301747264511\\
0.68	-0.12	15.6836365329385	15.6836365329385\\
0.7	-0.12	15.4117791291996	15.4117791291996\\
0.72	-0.12	15.1154331981308	15.1154331981308\\
0.74	-0.12	14.7958747614468	14.7958747614468\\
0.76	-0.12	14.4541849580099	14.4541849580099\\
0.78	-0.12	14.091143403936	14.091143403936\\
0.8	-0.12	13.7074435779581	13.7074435779581\\
0.2	-0.1	13.5580251993736	13.5580251993736\\
0.22	-0.1	13.9464696794638	13.9464696794638\\
0.24	-0.1	14.3131015221091	14.3131015221091\\
0.26	-0.1	14.6564191146348	14.6564191146348\\
0.28	-0.1	14.975085285284	14.975085285284\\
0.3	-0.1	15.2680369812328	15.2680369812328\\
0.32	-0.1	15.534535862064	15.534535862064\\
0.34	-0.1	15.7739853790561	15.7739853790561\\
0.36	-0.1	15.9858178910384	15.9858178910384\\
0.38	-0.1	16.169329250409	16.169329250409\\
0.4	-0.1	16.3237792905861	16.3237792905861\\
0.42	-0.1	16.4490180226271	16.4490180226271\\
0.44	-0.1	16.545033880084	16.545033880084\\
0.46	-0.1	16.6115782709025	16.6115782709025\\
0.48	-0.1	16.6484427647626	16.6484427647626\\
0.5	-0.1	16.6555012565634	16.6555012565634\\
0.52	-0.1	16.6328313817325	16.6328313817325\\
0.54	-0.1	16.5807317135784	16.5807317135784\\
0.56	-0.1	16.499330265725	16.499330265725\\
0.58	-0.1	16.3888855361034	16.3888855361034\\
0.6	-0.1	16.2497197668237	16.2497197668237\\
0.62	-0.1	16.0823150998178	16.0823150998178\\
0.64	-0.1	15.8876304040833	15.8876304040833\\
0.66	-0.1	15.666441607696	15.666441607696\\
0.68	-0.1	15.4194234407071	15.4194234407071\\
0.7	-0.1	15.1470033475458	15.1470033475458\\
0.72	-0.1	14.8501120809671	14.8501120809671\\
0.74	-0.1	14.5300605637591	14.5300605637591\\
0.76	-0.1	14.1878253943866	14.1878253943866\\
0.78	-0.1	13.8242407639412	13.8242407639412\\
0.8	-0.1	13.439950223547	13.439950223547\\
0.2	-0.08	13.3354466612777	13.3354466612777\\
0.22	-0.08	13.724437290038	13.724437290038\\
0.24	-0.08	14.0915902942937	14.0915902942937\\
0.26	-0.08	14.4353703286807	14.4353703286807\\
0.28	-0.08	14.7544585906248	14.7544585906248\\
0.3	-0.08	15.0478175593047	15.0478175593047\\
0.32	-0.08	15.3147045965957	15.3147045965957\\
0.34	-0.08	15.5545499212985	15.5545499212985\\
0.36	-0.08	15.7668299101663	15.7668299101663\\
0.38	-0.08	15.950782170275	15.950782170275\\
0.4	-0.08	16.1056612002987	16.1056612002987\\
0.42	-0.08	16.2313000195771	16.2313000195771\\
0.44	-0.08	16.3276907287854	16.3276907287854\\
0.46	-0.08	16.3945367773136	16.3945367773136\\
0.48	-0.08	16.4316034940824	16.4316034940824\\
0.5	-0.08	16.4387547369034	16.4387547369034\\
0.52	-0.08	16.4161630838761	16.4161630838761\\
0.54	-0.08	16.3640418960242	16.3640418960242\\
0.56	-0.08	16.2825449140692	16.2825449140692\\
0.58	-0.08	16.1719274614258	16.1719274614258\\
0.6	-0.08	16.0325094256961	16.0325094256961\\
0.62	-0.08	15.8648332433903	15.8648332433903\\
0.64	-0.08	15.6698486421414	15.6698486421414\\
0.66	-0.08	15.4482726085366	15.4482726085366\\
0.68	-0.08	15.2008043312425	15.2008043312425\\
0.7	-0.08	14.9279073615943	14.9279073615943\\
0.72	-0.08	14.6305884390715	14.6305884390715\\
0.74	-0.08	14.3101653446816	14.3101653446816\\
0.76	-0.08	13.9675200115297	13.9675200115297\\
0.78	-0.08	13.6035509412477	13.6035509412477\\
0.8	-0.08	13.2187875397393	13.2187875397393\\
0.2	-0.06	13.1594016757247	13.1594016757247\\
0.22	-0.06	13.5487801231364	13.5487801231364\\
0.24	-0.06	13.9163208604341	13.9163208604341\\
0.26	-0.06	14.2604258506414	14.2604258506414\\
0.28	-0.06	14.5798067097512	14.5798067097512\\
0.3	-0.06	14.8734712593739	14.8734712593739\\
0.32	-0.06	15.1406481851504	15.1406481851504\\
0.34	-0.06	15.3808474698988	15.3808474698988\\
0.36	-0.06	15.5934861609676	15.5934861609676\\
0.38	-0.06	15.7777749231369	15.7777749231369\\
0.4	-0.06	15.9330216896321	15.9330216896321\\
0.42	-0.06	16.0590262542122	16.0590262542122\\
0.44	-0.06	16.1557612593813	16.1557612593813\\
0.46	-0.06	16.2228930838588	16.2228930838588\\
0.48	-0.06	16.260137842577	16.260137842577\\
0.5	-0.06	16.267399426277	16.267399426277\\
0.52	-0.06	16.2448836008698	16.2448836008698\\
0.54	-0.06	16.1927727226915	16.1927727226915\\
0.56	-0.06	16.1112170835598	16.1112170835598\\
0.58	-0.06	16.0004818949036	16.0004818949036\\
0.6	-0.06	15.8608732733953	15.8608732733953\\
0.62	-0.06	15.6930097016573	15.6930097016573\\
0.64	-0.06	15.4977901699655	15.4977901699655\\
0.66	-0.06	15.2759012276269	15.2759012276269\\
0.68	-0.06	15.0280348263777	15.0280348263777\\
0.7	-0.06	14.7547488852449	14.7547488852449\\
0.72	-0.06	14.4571424402705	14.4571424402705\\
0.74	-0.06	14.1364667037148	14.1364667037148\\
0.76	-0.06	13.7935744310353	13.7935744310353\\
0.78	-0.06	13.4293368666418	13.4293368666418\\
0.8	-0.06	13.04424386499	13.04424386499\\
0.2	-0.04	13.0301008540504	13.0301008540504\\
0.22	-0.04	13.4196984761798	13.4196984761798\\
0.24	-0.04	13.7874858491628	13.7874858491628\\
0.26	-0.04	14.1317944504799	14.1317944504799\\
0.28	-0.04	14.4513401630914	14.4513401630914\\
0.3	-0.04	14.7451946501691	14.7451946501691\\
0.32	-0.04	15.0125912798587	15.0125912798587\\
0.34	-0.04	15.2530757575496	15.2530757575496\\
0.36	-0.04	15.4659811680366	15.4659811680366\\
0.38	-0.04	15.6505251663039	15.6505251663039\\
0.4	-0.04	15.8060784249523	15.8060784249523\\
0.42	-0.04	15.932411226264	15.932411226264\\
0.44	-0.04	16.0294863785076	16.0294863785076\\
0.46	-0.04	16.0968715636101	16.0968715636101\\
0.48	-0.04	16.1342638808896	16.1342638808896\\
0.5	-0.04	16.1416422169148	16.1416422169148\\
0.52	-0.04	16.1192080136857	16.1192080136857\\
0.54	-0.04	16.0671232102657	16.0671232102657\\
0.56	-0.04	15.9855563471934	15.9855563471934\\
0.58	-0.04	15.8747517845656	15.8747517845656\\
0.6	-0.04	15.735024440999	15.735024440999\\
0.62	-0.04	15.5670465810174	15.5670465810174\\
0.64	-0.04	15.3716497758706	15.3716497758706\\
0.66	-0.04	15.1495329529541	15.1495329529541\\
0.68	-0.04	14.9013577043199	14.9013577043199\\
0.7	-0.04	14.6277679490221	14.6277679490221\\
0.72	-0.04	14.330005242367	14.330005242367\\
0.74	-0.04	14.0092151687613	14.0092151687613\\
0.76	-0.04	13.6662162303854	13.6662162303854\\
0.78	-0.04	13.3018201024186	13.3018201024186\\
0.8	-0.04	12.9165412211957	12.9165412211957\\
0.2	-0.02	12.9477081124841	12.9477081124841\\
0.22	-0.02	13.3373665470553	13.3373665470553\\
0.24	-0.02	13.7052300406882	13.7052300406882\\
0.26	-0.02	14.0496239875741	14.0496239875741\\
0.28	-0.02	14.3692346947096	14.3692346947096\\
0.3	-0.02	14.6631846168958	14.6631846168958\\
0.32	-0.02	14.9307095979004	14.9307095979004\\
0.34	-0.02	15.1713839172122	15.1713839172122\\
0.36	-0.02	15.384482534275	15.384482534275\\
0.38	-0.02	15.5691956558336	15.5691956558336\\
0.4	-0.02	15.7249979273812	15.7249979273812\\
0.42	-0.02	15.8516324236719	15.8516324236719\\
0.44	-0.02	15.9490142599708	15.9490142599708\\
0.46	-0.02	16.0166025897387	16.0166025897387\\
0.48	-0.02	16.054127309408	16.054127309408\\
0.5	-0.02	16.0616349709714	16.0616349709714\\
0.52	-0.02	16.0392852901507	16.0392852901507\\
0.54	-0.02	15.9872644048506	15.9872644048506\\
0.56	-0.02	15.905727283006	15.905727283006\\
0.58	-0.02	15.7949146918339	15.7949146918339\\
0.6	-0.02	15.6551193752761	15.6551193752761\\
0.62	-0.02	15.4870918190392	15.4870918190392\\
0.64	-0.02	15.2916122258303	15.2916122258303\\
0.66	-0.02	15.0693346073673	15.0693346073673\\
0.68	-0.02	14.8209309610906	14.8209309610906\\
0.7	-0.02	14.5471627289954	14.5471627289954\\
0.72	-0.02	14.2493581437022	14.2493581437022\\
0.74	-0.02	13.9285873068511	13.9285873068511\\
0.76	-0.02	13.5855907643354	13.5855907643354\\
0.78	-0.02	13.2211514362373	13.2211514362373\\
0.8	-0.02	12.8358203292802	12.8358203292802\\
0.2	0	12.912331265074	12.912331265074\\
0.22	0	13.3019117063117	13.3019117063117\\
0.24	0	13.6696908876087	13.6696908876087\\
0.26	0	14.0140579449206	14.0140579449206\\
0.28	0	14.3336274801086	14.3336274801086\\
0.3	0	14.6275816940795	14.6275816940795\\
0.32	0	14.8951528174031	14.8951528174031\\
0.34	0	15.135907903392	15.135907903392\\
0.36	0	15.349116500556	15.349116500556\\
0.38	0	15.533922521633	15.533922521633\\
0.4	0	15.6898904467555	15.6898904467555\\
0.42	0	15.8167891826088	15.8167891826088\\
0.44	0	15.9144305512199	15.9144305512199\\
0.46	0	15.9821811356159	15.9821811356159\\
0.48	0	16.0198430629345	16.0198430629345\\
0.5	0	16.0275040023694	16.0275040023694\\
0.52	0	16.0052455172516	16.0052455172516\\
0.54	0	15.9533245551352	15.9533245551352\\
0.56	0	15.8718466608152	15.8718466608152\\
0.58	0	15.7610621656337	15.7610621656337\\
0.6	0	15.6212757423347	15.6212757423347\\
0.62	0	15.453267404411	15.453267404411\\
0.64	0	15.2577877786978	15.2577877786978\\
0.66	0	15.0354261500276	15.0354261500276\\
0.68	0	14.786906514586	14.786906514586\\
0.7	0	14.5130748859603	14.5130748859603\\
0.72	0	14.215328810613	14.215328810613\\
0.74	0	13.8946716380783	13.8946716380783\\
0.76	0	13.551783425531	13.551783425531\\
0.78	0	13.1874210559106	13.1874210559106\\
0.8	0	12.8021736971779	12.8021736971779\\
0.2	0.02	12.9240399134137	12.9240399134137\\
0.22	0.02	13.3134168141473	13.3134168141473\\
0.24	0.02	13.6809856591048	13.6809856591048\\
0.26	0.02	14.0251927405248	14.0251927405248\\
0.28	0.02	14.3446058803816	14.3446058803816\\
0.3	0.02	14.6384663717184	14.6384663717184\\
0.32	0.02	14.9060122193715	14.9060122193715\\
0.34	0.02	15.1467288414562	15.1467288414562\\
0.36	0.02	15.3599526440095	15.3599526440095\\
0.38	0.02	15.5447864442473	15.5447864442473\\
0.4	0.02	15.7008507519875	15.7008507519875\\
0.42	0.02	15.8279296710741	15.8279296710741\\
0.44	0.02	15.925747568887	15.925747568887\\
0.46	0.02	15.9936360966975	15.9936360966975\\
0.48	0.02	16.0314839098105	16.0314839098105\\
0.5	0.02	16.0393088967297	16.0393088967297\\
0.52	0.02	16.0171592629725	16.0171592629725\\
0.54	0.02	15.965360363563	15.965360363563\\
0.56	0.02	15.8839522996072	15.8839522996072\\
0.58	0.02	15.7732525644202	15.7732525644202\\
0.6	0.02	15.633554601707	15.633554601707\\
0.62	0.02	15.4656321740137	15.4656321740137\\
0.64	0.02	15.2702143256841	15.2702143256841\\
0.66	0.02	15.0478683911681	15.0478683911681\\
0.68	0.02	14.7993477014588	14.7993477014588\\
0.7	0.02	14.5255779271551	14.5255779271551\\
0.72	0.02	14.2279893783933	14.2279893783933\\
0.74	0.02	13.9075278608451	13.9075278608451\\
0.76	0.02	13.5648334649074	13.5648334649074\\
0.78	0.02	13.2006620579277	13.2006620579277\\
0.8	0.02	12.815665423277	12.815665423277\\
0.2	0.04	12.9828685048719	12.9828685048719\\
0.22	0.04	13.3719177000735	13.3719177000735\\
0.24	0.04	13.7391418281863	13.7391418281863\\
0.26	0.04	14.0830496353589	14.0830496353589\\
0.28	0.04	14.4022063883061	14.4022063883061\\
0.3	0.04	14.6958609542177	14.6958609542177\\
0.32	0.04	14.9632881049908	14.9632881049908\\
0.34	0.04	15.2038738542249	15.2038738542249\\
0.36	0.04	15.4169910480549	15.4169910480549\\
0.38	0.04	15.6017903146691	15.6017903146691\\
0.4	0.04	15.7578989133512	15.7578989133512\\
0.42	0.04	15.8850620190089	15.8850620190089\\
0.44	0.04	15.9829634675329	15.9829634675329\\
0.46	0.04	16.0509889751528	16.0509889751528\\
0.48	0.04	16.0890334344358	16.0890334344358\\
0.5	0.04	16.0970274180816	16.0970274180816\\
0.52	0.04	16.0750214919073	16.0750214919073\\
0.54	0.04	16.0233513978126	16.0233513978126\\
0.56	0.04	15.9420565767132	15.9420565767132\\
0.58	0.04	15.8315029218318	15.8315029218318\\
0.6	0.04	15.6919621198841	15.6919621198841\\
0.62	0.04	15.5242135474406	15.5242135474406\\
0.64	0.04	15.3288967498168	15.3288967498168\\
0.66	0.04	15.106634643657	15.106634643657\\
0.68	0.04	14.85825876418	14.85825876418\\
0.7	0.04	14.5846977284148	14.5846977284148\\
0.72	0.04	14.2873559777789	14.2873559777789\\
0.74	0.04	13.9671672363536	13.9671672363536\\
0.76	0.04	13.6247469676119	13.6247469676119\\
0.78	0.04	13.2608834078128	13.2608834078128\\
0.8	0.04	12.876277882178	12.876277882178\\
0.2	0.06	13.088783417309	13.088783417309\\
0.22	0.06	13.4773686196884	13.4773686196884\\
0.24	0.06	13.8441270308206	13.8441270308206\\
0.26	0.06	14.1876136066024	14.1876136066024\\
0.28	0.06	14.5064140137053	14.5064140137053\\
0.3	0.06	14.7997299844244	14.7997299844244\\
0.32	0.06	15.0669269920337	15.0669269920337\\
0.34	0.06	15.3073085681467	15.3073085681467\\
0.36	0.06	15.5202017539912	15.5202017539912\\
0.38	0.06	15.704874548137	15.704874548137\\
0.4	0.06	15.8609768118457	15.8609768118457\\
0.42	0.06	15.9881557749518	15.9881557749518\\
0.44	0.06	16.0860700928811	16.0860700928811\\
0.46	0.06	16.1542134668443	16.1542134668443\\
0.48	0.06	16.1924174613132	16.1924174613132\\
0.5	0.06	16.2005852553802	16.2005852553802\\
0.52	0.06	16.1787519737888	16.1787519737888\\
0.54	0.06	16.1272424123335	16.1272424123335\\
0.56	0.06	16.0461088525252	16.0461088525252\\
0.58	0.06	15.935768102714	15.935768102714\\
0.6	0.06	15.7964594824377	15.7964594824377\\
0.62	0.06	15.6289741813653	15.6289741813653\\
0.64	0.06	15.4338099959988	15.4338099959988\\
0.66	0.06	15.211688311137	15.211688311137\\
0.68	0.06	14.9635777318451	14.9635777318451\\
0.7	0.06	14.6903678813435	14.6903678813435\\
0.72	0.06	14.3933664517384	14.3933664517384\\
0.74	0.06	14.073525257865	14.073525257865\\
0.76	0.06	13.7314714649573	13.7314714649573\\
0.78	0.06	13.36801919023	13.36801919023\\
0.8	0.06	12.9839453184428	12.9839453184428\\
0.2	0.08	13.2416829624164	13.2416829624164\\
0.22	0.08	13.6296563536501	13.6296563536501\\
0.24	0.08	13.9958187546023	13.9958187546023\\
0.26	0.08	14.3387769024641	14.3387769024641\\
0.28	0.08	14.6571213853757	14.6571213853757\\
0.3	0.08	14.9500016452455	14.9500016452455\\
0.32	0.08	15.2168274544904	15.2168274544904\\
0.34	0.08	15.45692618783	15.45692618783\\
0.36	0.08	15.6695242828686	15.6695242828686\\
0.38	0.08	15.8539782665825	15.8539782665825\\
0.4	0.08	16.0099969276605	16.0099969276605\\
0.42	0.08	16.1371566509654	16.1371566509654\\
0.44	0.08	16.2350476042114	16.2350476042114\\
0.46	0.08	16.3032605026187	16.3032605026187\\
0.48	0.08	16.3415725759716	16.3415725759716\\
0.5	0.08	16.3498928725849	16.3498928725849\\
0.52	0.08	16.3282583051384	16.3282583051384\\
0.54	0.08	16.2769389559276	16.2769389559276\\
0.56	0.08	16.1960383840203	16.1960383840203\\
0.58	0.08	16.0859626838588	16.0859626838588\\
0.6	0.08	15.9469739649996	15.9469739649996\\
0.62	0.08	15.7797844739034	15.7797844739034\\
0.64	0.08	15.5848665330303	15.5848665330303\\
0.66	0.08	15.3629547726022	15.3629547726022\\
0.68	0.08	15.1152034448755	15.1152034448755\\
0.7	0.08	14.8424488578281	14.8424488578281\\
0.72	0.08	14.5459000969556	14.5459000969556\\
0.74	0.08	14.2264972402392	14.2264972402392\\
0.76	0.08	13.8849025380355	13.8849025380355\\
0.78	0.08	13.5219859866258	13.5219859866258\\
0.8	0.08	13.1385238601648	13.1385238601648\\
0.2	0.1	13.4414193610402	13.4414193610402\\
0.22	0.1	13.8286390507542	13.8286390507542\\
0.24	0.1	14.1940474775077	14.1940474775077\\
0.26	0.1	14.5363669436148	14.5363669436148\\
0.28	0.1	14.8541764343387	14.8541764343387\\
0.3	0.1	15.1465335816582	15.1465335816582\\
0.32	0.1	15.4128824168075	15.4128824168075\\
0.34	0.1	15.6525898867638	15.6525898867638\\
0.36	0.1	15.8648313982753	15.8648313982753\\
0.38	0.1	16.0489924344811	16.0489924344811\\
0.4	0.1	16.204840596653	16.204840596653\\
0.42	0.1	16.3319123241398	16.3319123241398\\
0.44	0.1	16.4297586803526	16.4297586803526\\
0.46	0.1	16.4980113831452	16.4980113831452\\
0.48	0.1	16.5363837114304	16.5363837114304\\
0.5	0.1	16.5448351629497	16.5448351629497\\
0.52	0.1	16.5233993137574	16.5233993137574\\
0.54	0.1	16.4723250847963	16.4723250847963\\
0.56	0.1	16.3917163247259	16.3917163247259\\
0.58	0.1	16.2819439756124	16.2819439756124\\
0.6	0.1	16.1433252759744	16.1433252759744\\
0.62	0.1	15.9764865288574	15.9764865288574\\
0.64	0.1	15.7819039336255	15.7819039336255\\
0.66	0.1	15.5603282609358	15.5603282609358\\
0.68	0.1	15.3129932603195	15.3129932603195\\
0.7	0.1	15.0407557641074	15.0407557641074\\
0.72	0.1	14.744790259945	14.744790259945\\
0.74	0.1	14.4259271263899	14.4259271263899\\
0.76	0.1	14.0848757537623	14.0848757537623\\
0.78	0.1	13.7225864681329	13.7225864681329\\
0.8	0.1	13.33985145594	13.33985145594\\
0.2	0.12	13.6877819345175	13.6877819345175\\
0.22	0.12	14.0741136872976	14.0741136872976\\
0.24	0.12	14.438640935172	14.438640935172\\
0.26	0.12	14.7802030394835	14.7802030394835\\
0.28	0.12	15.0973799760507	15.0973799760507\\
0.3	0.12	15.3891460857939	15.3891460857939\\
0.32	0.12	15.6549252911693	15.6549252911693\\
0.34	0.12	15.8941207677178	15.8941207677178\\
0.36	0.12	16.1059290693106	16.1059290693106\\
0.38	0.12	16.2897462097182	16.2897462097182\\
0.4	0.12	16.4453369712325	16.4453369712325\\
0.42	0.12	16.5722431881935	16.5722431881935\\
0.44	0.12	16.6700015684925	16.6700015684925\\
0.46	0.12	16.7382688534816	16.7382688534816\\
0.48	0.12	16.7766723710256	16.7766723710256\\
0.5	0.12	16.7852405354406	16.7852405354406\\
0.52	0.12	16.7640176404065	16.7640176404065\\
0.54	0.12	16.7132060224727	16.7132060224727\\
0.56	0.12	16.6329438963145	16.6329438963145\\
0.58	0.12	16.5235186881026	16.5235186881026\\
0.6	0.12	16.3853029357219	16.3853029357219\\
0.62	0.12	16.2188862576082	16.2188862576082\\
0.64	0.12	16.0247155828682	16.0247155828682\\
0.66	0.12	15.8035982858535	15.8035982858535\\
0.68	0.12	15.5567525168199	15.5567525168199\\
0.7	0.12	15.2850924874024	15.2850924874024\\
0.72	0.12	14.9897963609934	14.9897963609934\\
0.74	0.12	14.6715788214712	14.6715788214712\\
0.76	0.12	14.3311682864513	14.3311682864513\\
0.78	0.12	13.9695968184361	13.9695968184361\\
0.8	0.12	13.5876902245425	13.5876902245425\\
0.2	0.14	13.980503419843	13.980503419843\\
0.22	0.14	14.3658044425551	14.3658044425551\\
0.24	0.14	14.7293673986635	14.7293673986635\\
0.26	0.14	15.0700609561257	15.0700609561257\\
0.28	0.14	15.3864843421336	15.3864843421336\\
0.3	0.14	15.6775630834179	15.6775630834179\\
0.32	0.14	15.9426832468221	15.9426832468221\\
0.34	0.14	16.1812691658977	16.1812691658977\\
0.36	0.14	16.3925655657633	16.3925655657633\\
0.38	0.14	16.5760019839934	16.5760019839934\\
0.4	0.14	16.7312645699945	16.7312645699945\\
0.42	0.14	16.8579466656674	16.8579466656674\\
0.44	0.14	16.9555632442676	16.9555632442676\\
0.46	0.14	17.023784186111	17.023784186111\\
0.48	0.14	17.0621966169518	17.0621966169518\\
0.5	0.14	17.0708711370556	17.0708711370556\\
0.52	0.14	17.0498777969228	17.0498777969228\\
0.54	0.14	16.9993540163683	16.9993540163683\\
0.56	0.14	16.9194537499582	16.9194537499582\\
0.58	0.14	16.8104180782684	16.8104180782684\\
0.6	0.14	16.6726316080641	16.6726316080641\\
0.62	0.14	16.5066888956963	16.5066888956963\\
0.64	0.14	16.3130201642762	16.3130201642762\\
0.66	0.14	16.0924828020277	16.0924828020277\\
0.68	0.14	15.8462006185388	15.8462006185388\\
0.7	0.14	15.5752041297984	15.5752041297984\\
0.72	0.14	15.2806494621106	15.2806494621106\\
0.74	0.14	14.9631908827117	14.9631908827117\\
0.76	0.14	14.6235420631634	14.6235420631634\\
0.78	0.14	14.2627842906896	14.2627842906896\\
0.8	0.14	13.881771179273	13.881771179273\\
0.2	0.16	14.3192670255132	14.3192670255132\\
0.22	0.16	14.7034058530346	14.7034058530346\\
0.24	0.16	15.0659220136864	15.0659220136864\\
0.26	0.16	15.4056407672612	15.4056407672612\\
0.28	0.16	15.7212074740464	15.7212074740464\\
0.3	0.16	16.0114673748711	16.0114673748711\\
0.32	0.16	16.2758306063655	16.2758306063655\\
0.34	0.16	16.5137294293096	16.5137294293096\\
0.36	0.16	16.724458397917	16.724458397917\\
0.38	0.16	16.907454499662	16.907454499662\\
0.4	0.16	17.0623612941339	17.0623612941339\\
0.42	0.16	17.1887499388934	17.1887499388934\\
0.44	0.16	17.2861820920039	17.2861820920039\\
0.46	0.16	17.354274882394	17.354274882394\\
0.48	0.16	17.3926915806833	17.3926915806833\\
0.5	0.16	17.4014397083247	17.4014397083247\\
0.52	0.16	17.3806720586247	17.3806720586247\\
0.54	0.16	17.3304581845431	17.3304581845431\\
0.56	0.16	17.2509343667629	17.2509343667629\\
0.58	0.16	17.1423160365247	17.1423160365247\\
0.6	0.16	17.0050024770616	17.0050024770616\\
0.62	0.16	16.8395896619167	16.8395896619167\\
0.64	0.16	16.6464889204154	16.6464889204154\\
0.66	0.16	16.4266447643028	16.4266447643028\\
0.68	0.16	16.1810234440371	16.1810234440371\\
0.7	0.16	15.9107720553928	15.9107720553928\\
0.72	0.16	15.6170337768223	15.6170337768223\\
0.74	0.16	15.3004408065605	15.3004408065605\\
0.76	0.16	14.9616704521901	14.9616704521901\\
0.78	0.16	14.6018131756933	14.6018131756933\\
0.8	0.16	14.2217967481431	14.2217967481431\\
0.2	0.18	14.703710563087	14.703710563087\\
0.22	0.18	15.0865838837277	15.0865838837277\\
0.24	0.18	15.4479474686949	15.4479474686949\\
0.26	0.18	15.7866101454069	15.7866101454069\\
0.28	0.18	16.1012041979084	16.1012041979084\\
0.3	0.18	16.390518884703	16.390518884703\\
0.32	0.18	16.6540255682251	16.6540255682251\\
0.34	0.18	16.8911778220714	16.8911778220714\\
0.36	0.18	17.101272980904	17.101272980904\\
0.38	0.18	17.2837730510407	17.2837730510407\\
0.4	0.18	17.4382756749116	17.4382756749116\\
0.42	0.18	17.5642948122224	17.5642948122224\\
0.44	0.18	17.6614851519125	17.6614851519125\\
0.46	0.18	17.7294042009729	17.7294042009729\\
0.48	0.18	17.7677892414631	17.7677892414631\\
0.5	0.18	17.7766152189572	17.7766152189572\\
0.52	0.18	17.7560616116586	17.7560616116586\\
0.54	0.18	17.7061608505632	17.7061608505632\\
0.56	0.18	17.6270481184042	17.6270481184042\\
0.58	0.18	17.5188768493384	17.5188768493384\\
0.6	0.18	17.3820792503383	17.3820792503383\\
0.62	0.18	17.2172296218524	17.2172296218524\\
0.64	0.18	17.0247852009601	17.0247852009601\\
0.66	0.18	16.8057122736271	16.8057122736271\\
0.68	0.18	16.5608771723614	16.5608771723614\\
0.7	0.18	16.2914548992381	16.2914548992381\\
0.72	0.18	15.9985954728671	15.9985954728671\\
0.74	0.18	15.6829739729747	15.6829739729747\\
0.76	0.18	15.3451651349271	15.3451651349271\\
0.78	0.18	14.9863327760268	14.9863327760268\\
0.8	0.18	14.6074282103053	14.6074282103053\\
0.2	0.2	15.1334318922537	15.1334318922537\\
0.22	0.2	15.5149394836327	15.5149394836327\\
0.24	0.2	15.8750463432973	15.8750463432973\\
0.26	0.2	16.2125582146043	16.2125582146043\\
0.28	0.2	16.5260460031196	16.5260460031196\\
0.3	0.2	16.8143156578154	16.8143156578154\\
0.32	0.2	17.0768858685861	17.0768858685861\\
0.34	0.2	17.3132271327523	17.3132271327523\\
0.36	0.2	17.5225974500066	17.5225974500066\\
0.38	0.2	17.7045431019536	17.7045431019536\\
0.4	0.2	17.858556623669	17.858556623669\\
0.42	0.2	17.9841668211621	17.9841668211621\\
0.44	0.2	18.0810578474666	18.0810578474666\\
0.46	0.2	18.148771338953	18.148771338953\\
0.48	0.2	18.1870993855766	18.1870993855766\\
0.5	0.2	18.1960167458313	18.1960167458313\\
0.52	0.2	18.1756672094761	18.1756672094761\\
0.54	0.2	18.1260685865879	18.1260685865879\\
0.56	0.2	18.0473872551768	18.0473872551768\\
0.58	0.2	17.9396960750215	17.9396960750215\\
0.6	0.2	17.8034568429631	17.8034568429631\\
0.62	0.2	17.6392113305709	17.6392113305709\\
0.64	0.2	17.4475158129468	17.4475158129468\\
0.66	0.2	17.2292781187189	17.2292781187189\\
0.68	0.2	16.985325190776	16.985325190776\\
0.7	0.2	16.7168272791895	16.7168272791895\\
0.72	0.2	16.4249486854965	16.4249486854965\\
0.74	0.2	16.1103668886111	16.1103668886111\\
0.76	0.2	15.7736315346608	15.7736315346608\\
0.78	0.2	15.4159331500024	15.4159331500024\\
0.8	0.2	15.0382638127721	15.0382638127721\\
0.2	0.22	15.6079738541353	15.6079738541353\\
0.22	0.22	15.9880188435098	15.9880188435098\\
0.24	0.22	16.3467622059697	16.3467622059697\\
0.26	0.22	16.682997643105	16.682997643105\\
0.28	0.22	16.9952606721633	16.9952606721633\\
0.3	0.22	17.2824260507835	17.2824260507835\\
0.32	0.22	17.5439660911081	17.5439660911081\\
0.34	0.22	17.7794146496633	17.7794146496633\\
0.36	0.22	17.9880025687303	17.9880025687303\\
0.38	0.22	18.1692973608969	18.1692973608969\\
0.4	0.22	18.3227358675146	18.3227358675146\\
0.42	0.22	18.4479087312728	18.4479087312728\\
0.44	0.22	18.5444536960013	18.5444536960013\\
0.46	0.22	18.6119415921012	18.6119415921012\\
0.48	0.22	18.6502018450707	18.6502018450707\\
0.5	0.22	18.6592108610668	18.6592108610668\\
0.52	0.22	18.6390358849701	18.6390358849701\\
0.54	0.22	18.5897506812036	18.5897506812036\\
0.56	0.22	18.5114926078192	18.5114926078192\\
0.58	0.22	18.4043368992166	18.4043368992166\\
0.6	0.22	18.2687062217714	18.2687062217714\\
0.62	0.22	18.1051120399962	18.1051120399962\\
0.64	0.22	17.914225500911	17.914225500911\\
0.66	0.22	17.6968692316244	17.6968692316244\\
0.68	0.22	17.4538915569343	17.4538915569343\\
0.7	0.22	17.1864137514349	17.1864137514349\\
0.72	0.22	16.8956051989824	16.8956051989824\\
0.74	0.22	16.5821563665149	16.5821563665149\\
0.76	0.22	16.2466111643013	16.2466111643013\\
0.78	0.22	15.8901490256071	15.8901490256071\\
0.8	0.22	15.5138221852786	15.5138221852786\\
0.2	0.24	16.1268205683143	16.1268205683143\\
0.22	0.24	16.5053099136138	16.5053099136138\\
0.24	0.24	16.8625719967198	16.8625719967198\\
0.26	0.24	17.1974033456703	17.1974033456703\\
0.28	0.24	17.5083455107593	17.5083455107593\\
0.3	0.24	17.7943296232325	17.7943296232325\\
0.32	0.24	18.0547715056383	18.0547715056383\\
0.34	0.24	18.2892547396086	18.2892547396086\\
0.36	0.24	18.4970126441864	18.4970126441864\\
0.38	0.24	18.6775439624389	18.6775439624389\\
0.4	0.24	18.8303390612388	18.8303390612388\\
0.42	0.24	18.9550314579255	18.9550314579255\\
0.44	0.24	19.0511802614525	19.0511802614525\\
0.46	0.24	19.1184110031088	19.1184110031088\\
0.48	0.24	19.1565855347809	19.1565855347809\\
0.5	0.24	19.1656648582251	19.1656648582251\\
0.52	0.24	19.1456726066052	19.1456726066052\\
0.54	0.24	19.0967153874419	19.0967153874419\\
0.56	0.24	19.0188856032067	19.0188856032067\\
0.58	0.24	18.9122921794303	18.9122921794303\\
0.6	0.24	18.7773132057648	18.7773132057648\\
0.62	0.24	18.6144463050324	18.6144463050324\\
0.64	0.24	18.4244027040691	18.4244027040691\\
0.66	0.24	18.2080084192304	18.2080084192304\\
0.68	0.24	17.9660458351281	17.9660458351281\\
0.7	0.24	17.6996995709865	17.6996995709865\\
0.72	0.24	17.4100481843429	17.4100481843429\\
0.74	0.24	17.0978231465121	17.0978231465121\\
0.76	0.24	16.7635876676667	16.7635876676667\\
0.78	0.24	16.4084692172153	16.4084692172153\\
0.8	0.24	16.0335876788575	16.0335876788575\\
0.2	0.26	16.6893982708801	16.6893982708801\\
0.22	0.26	17.066227114665	17.066227114665\\
0.24	0.26	17.4218921892	17.4218921892\\
0.26	0.26	17.7552116281511	17.7552116281511\\
0.28	0.26	18.0647482343827	18.0647482343827\\
0.3	0.26	18.3494755951323	18.3494755951323\\
0.32	0.26	18.6087595919379	18.6087595919379\\
0.34	0.26	18.842202957019	18.842202957019\\
0.36	0.26	19.049053530164	19.049053530164\\
0.38	0.26	19.2287244284497	19.2287244284497\\
0.4	0.26	19.3808277958265	19.3808277958265\\
0.42	0.26	19.5049985431435	19.5049985431435\\
0.44	0.26	19.6006963518838	19.6006963518838\\
0.46	0.26	19.6676325666749	19.6676325666749\\
0.48	0.26	19.7056874161319	19.7056874161319\\
0.5	0.26	19.7148098781961	19.7148098781961\\
0.52	0.26	19.6950197112281	19.6950197112281\\
0.54	0.26	19.6464178079019	19.6464178079019\\
0.56	0.26	19.5690277551732	19.5690277551732\\
0.58	0.26	19.4629988415905	19.4629988415905\\
0.6	0.26	19.328700570638	19.328700570638\\
0.62	0.26	19.1666363487693	19.1666363487693\\
0.64	0.26	18.9775177769051	18.9775177769051\\
0.66	0.26	18.7621421187071	18.7621421187071\\
0.68	0.26	18.5212333163307	18.5212333163307\\
0.7	0.26	18.2560975799344	18.2560975799344\\
0.72	0.26	17.9677156436815	17.9677156436815\\
0.74	0.26	17.6568125604328	17.6568125604328\\
0.76	0.26	17.3239929551396	17.3239929551396\\
0.78	0.26	16.9703238876497	16.9703238876497\\
0.8	0.26	16.5970060808738	16.5970060808738\\
0.2	0.28	17.295104786981	17.295104786981\\
0.22	0.28	17.6701648962814	17.6701648962814\\
0.24	0.28	18.0241234285447	18.0241234285447\\
0.26	0.28	18.3558153556843	18.3558153556843\\
0.28	0.28	18.6638633390498	18.6638633390498\\
0.3	0.28	18.9472562927882	18.9472562927882\\
0.32	0.28	19.2053205108237	19.2053205108237\\
0.34	0.28	19.437648111999	19.437648111999\\
0.36	0.28	19.6434908646891	19.6434908646891\\
0.38	0.28	19.8222452248585	19.8222452248585\\
0.4	0.28	19.9735806558894	19.9735806558894\\
0.42	0.28	20.0971810634266	20.0971810634266\\
0.44	0.28	20.1923941128594	20.1923941128594\\
0.46	0.28	20.258996611923	20.258996611923\\
0.48	0.28	20.2968997749923	20.2968997749923\\
0.5	0.28	20.3060490745532	20.3060490745532\\
0.52	0.28	20.2864781399802	20.2864781399802\\
0.54	0.28	20.2382249435504	20.2382249435504\\
0.56	0.28	20.1612839084415	20.1612839084415\\
0.58	0.28	20.0558413182937	20.0558413182937\\
0.6	0.28	19.9222690756643	19.9222690756643\\
0.62	0.28	19.7610757138491	19.7610757138491\\
0.64	0.28	19.5729405569745	19.5729405569745\\
0.66	0.28	19.3586160063068	19.3586160063068\\
0.68	0.28	19.1188664239264	19.1188664239264\\
0.7	0.28	18.8549731371272	18.8549731371272\\
0.72	0.28	18.5679656524367	18.5679656524367\\
0.74	0.28	18.258484302644	18.258484302644\\
0.76	0.28	17.9271892779446	17.9271892779446\\
0.78	0.28	17.5751030522442	17.5751030522442\\
0.8	0.28	17.2034559788036	17.2034559788036\\
0.2	0.3	17.9432956517549	17.9432956517549\\
0.22	0.3	18.3164677905323	18.3164677905323\\
0.24	0.3	18.6685998913522	18.6685998913522\\
0.26	0.3	18.9985740658921	18.9985740658921\\
0.28	0.3	19.3050502602593	19.3050502602593\\
0.3	0.3	19.5870055177753	19.5870055177753\\
0.32	0.3	19.8437890744002	19.8437890744002\\
0.34	0.3	20.0749229114301	20.0749229114301\\
0.36	0.3	20.2796659582134	20.2796659582134\\
0.38	0.3	20.4574616521272	20.4574616521272\\
0.4	0.3	20.6079658831316	20.6079658831316\\
0.42	0.3	20.7309142027376	20.7309142027376\\
0.44	0.3	20.8256190539736	20.8256190539736\\
0.46	0.3	20.8918628780194	20.8918628780194\\
0.48	0.3	20.9295728759767	20.9295728759767\\
0.5	0.3	20.9387215840761	20.9387215840761\\
0.52	0.3	20.9193774249479	20.9193774249479\\
0.54	0.3	20.871453609703	20.871453609703\\
0.56	0.3	20.7949789579142	20.7949789579142\\
0.58	0.3	20.6901554544773	20.6901554544773\\
0.6	0.3	20.5573805532476	20.5573805532476\\
0.62	0.3	20.3970885791948	20.3970885791948\\
0.64	0.3	20.2099784625738	20.2099784625738\\
0.66	0.3	19.99673621999	19.99673621999\\
0.68	0.3	19.7582371453967	19.7582371453967\\
0.7	0.3	19.4957033208851	19.4957033208851\\
0.72	0.3	19.2101339461769	19.2101339461769\\
0.74	0.3	18.9021797245939	18.9021797245939\\
0.76	0.3	18.5725031306606	18.5725031306606\\
0.78	0.3	18.2221021771616	18.2221021771616\\
0.8	0.3	17.8522613865944	17.8522613865944\\
};

\addplot3 [color=mycolor1, dotted, line width=2.0pt]
 table[row sep=crcr] {%
0.5	-0.3	21.2404921720053\\
0.5	-0.28	20.5916247712227\\
0.5	-0.26	19.9834037537941\\
0.5	-0.24	19.4165403224433\\
0.5	-0.22	18.8916928863053\\
0.5	-0.2	18.4095141095484\\
0.5	-0.18	17.9705519878681\\
0.5	-0.16	17.5752643467509\\
0.5	-0.14	17.224063732732\\
0.5	-0.12	16.9173684750453\\
0.5	-0.1	16.6555012565634\\
0.5	-0.08	16.4387547369034\\
0.5	-0.06	16.267399426277\\
0.5	-0.04	16.1416422169148\\
0.5	-0.02	16.0616349709714\\
0.5	0	16.0275040023694\\
0.5	0.02	16.0393088967297\\
0.5	0.04	16.0970274180816\\
0.5	0.06	16.2005852553802\\
0.5	0.08	16.3498928725849\\
0.5	0.1	16.5448351629497\\
0.5	0.12	16.7852405354406\\
0.5	0.14	17.0708711370556\\
0.5	0.16	17.4014397083247\\
0.5	0.18	17.7766152189572\\
0.5	0.2	18.1960167458313\\
0.5	0.22	18.6592108610668\\
0.5	0.24	19.1656648582251\\
0.5	0.26	19.7148098781961\\
0.5	0.28	20.3060490745532\\
0.5	0.3	20.9387215840761\\
};
 \addlegendentry{$\mc S_{\mb \tau}^\perp$}

\addplot3 [color=mycolor2, dotted, line width=2.0pt]
 table[row sep=crcr] {%
0.2	0	12.912331265074\\
0.22	0	13.3019117063117\\
0.24	0	13.6696908876087\\
0.26	0	14.0140579449206\\
0.28	0	14.3336274801086\\
0.3	0	14.6275816940795\\
0.32	0	14.8951528174031\\
0.34	0	15.135907903392\\
0.36	0	15.349116500556\\
0.38	0	15.533922521633\\
0.4	0	15.6898904467555\\
0.42	0	15.8167891826088\\
0.44	0	15.9144305512199\\
0.46	0	15.9821811356159\\
0.48	0	16.0198430629345\\
0.5	0	16.0275040023694\\
0.52	0	16.0052455172516\\
0.54	0	15.9533245551352\\
0.56	0	15.8718466608152\\
0.58	0	15.7610621656337\\
0.6	0	15.6212757423347\\
0.62	0	15.453267404411\\
0.64	0	15.2577877786978\\
0.66	0	15.0354261500276\\
0.68	0	14.786906514586\\
0.7	0	14.5130748859603\\
0.72	0	14.215328810613\\
0.74	0	13.8946716380783\\
0.76	0	13.551783425531\\
0.78	0	13.1874210559106\\
0.8	0	12.8021736971779\\
};
 \addlegendentry{$\mc S_{\mb \tau}$}


\end{axis}

